Face Beautification: Beyond Makeup Transfer

Facial appearance plays an important role in our social lives. Subjective perception of women's beauty depends on various face-related (e.g., skin, shape, hair) and environmental (e.g., makeup, lighting, angle) factors. Similar to cosmetic surgery in the physical world, virtual face beautification is an emerging field with many open issues to be addressed. Inspired by the latest advances in style-based synthesis and face beauty prediction, we propose a novel framework of face beautification. For a given reference face with a high beauty score, our GAN-based architecture is capable of translating an inquiry face into a sequence of beautified face images with referenced beauty style and targeted beauty score values. To achieve this objective, we propose to integrate both style-based beauty representation (extracted from the reference face) and beauty score prediction (trained on SCUT-FBP database) into the process of beautification. Unlike makeup transfer, our approach targets at many-to-many (instead of one-to-one) translation where multiple outputs can be defined by either different references or varying beauty scores. Extensive experimental results are reported to demonstrate the effectiveness and flexibility of the proposed face beautification framework.

==> CCS_Keywords.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%

\begin{CCSXML}
    <ccs2012>
    <concept>
        <concept_id>10010147.10010178.10010224.10010245.10010254</concept_id>
        <concept_desc>Computing methodologies~Reconstruction</concept_desc>
        <concept_significance>500</concept_significance>
    </concept>
    <concept>
        <concept_id>10010147.10010257.10010293.10010294</concept_id>
        <concept_desc>Computing methodologies~Neural networks</concept_desc>
        <concept_significance>300</concept_significance>
    </concept>
    <concept>
        <concept_id>10010147.10010371.10010382</concept_id>
        <concept_desc>Computing methodologies~Image manipulation</concept_desc>
        <concept_significance>300</concept_significance>
    </concept>
    </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Reconstruction}
\ccsdesc[300]{Computing methodologies~Neural networks}
\ccsdesc[300]{Computing methodologies~Image manipulation}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Digital avatar reconstruction, texture synthesis, face representation optimization}


==> Section/Acknowledgments.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
%%\begin{acks}

%%\end{acks}


\begin{align}
    \textbf {E}_{c}
    \\
    \textbf {E}_{s}
    \\
    \textbf {S}_{a}
    \\
    \textbf {S}_{b}
    \\
    \textbf {C}_{b}
    \\
    \textbf {G}
    \\
    \textbf {A}
    \\
    \textbf {B}
    \\
    \textbf {AB}
    \\
    \textbf {A}^{\bf{'}}
    \\
    \textbf {B}^{{'}}
    \\
    \textbf {FC1}
    \\
    \textbf {FC2}
    \\
    \textbf {CNN}
    \\
    \textbf {Beauty Score}
    \\
    \textbf {Tuning}
    \\
    \textbf {LighCNN}
    \\
    \textbf {256}
    \\
    \textbf {8*8*128}
\end{align}
